Can AI writing be salvaged? Mitigating Idiosyncrasies and Improving Human-AI Alignment in the Writing Process through Edits

LLM-based applications are helping people write, and LLM-generated text is making its way into social media, journalism, and our classrooms. However, the differences between LLM-generated and human written text remain unclear. To explore this, we hired professional writers to edit paragraphs in several creative domains. We first found these writers agree on undesirable idiosyncrasies in LLM generated text, formalizing it into a seven-category taxonomy (e.g. clich\'es, unnecessary exposition). Second, we curated the LAMP corpus: 1,057 LLM-generated paragraphs edited by professional writers according to our taxonomy. Analysis of LAMP reveals that none of the LLMs used in our study (GPT4o, Claude-3.5-Sonnet, Llama-3.1-70b) outperform each other in terms of writing quality, revealing common limitations across model families. Third, building on existing work in automatic editing we evaluated methods to improve LLM-generated text. A large-scale preference annotation confirms that although experts largely prefer text edited by other experts, automatic editing methods show promise in improving alignment between LLM-generated and human-written text.

==> tables/table_source.tex <==
\begin{table*}[!ht]
\small
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{|l|c|l|l|}
\hline
Domain                                & Source \& Genre                                                            & Example Paragraph                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                & \#N \\ \hline
Fiction                               & \begin{tabular}[c]{@{}l@{}}\href{https://www.newyorker.com/fiction-and-poetry}{The NewYorker}\\ (Literary Fiction)\end{tabular} & \begin{tabular}[c]{@{}l@{}}The sunset is a red-gold rumpus on the western sky. It has rained. The crow tosses itself \\ from branch to branch, pole to pole, glistening on its pace, and she follows. They are soon\\ far from where they began, streets unfamiliar to her, an older part of town, crossed by alleys\\ where forms flit. There is the stillness after rain. Rank risings rise. Trees drip. Street lamps \\ loom. Night takes on a polish, a pure power. She glances into windows as she goes. Blaze \\ of an empty kitchen. A man reading. Old Christmas tree in a corner. It  feels secret. The sky\\  is clearing overhead. She feels secret, too. She feels tremendous.\end{tabular}                                                                                                                                                                          & 815   \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}Creative \\Non-Fiction\end{tabular}} & \begin{tabular}[c]{@{}l@{}}\href{https://www.nytimes.com/column/36-hours}{NYTimes}\\ (Travel Writing)\end{tabular}         & \begin{tabular}[c]{@{}l@{}}Prague, the Czech capital, is finding a new balance between preserving its past and\\ embracing the future, improving many of its important historic sites while making striking \\ additions to its skyline. A reset on tourism during the pandemic has left the city feeling \\ more focused on local residents, with many new parks, bike trails, pedestrian bridges \& \\ other amenities showing up outside the historic center. The best new cafes, bars and \\ restaurants, as well, are often found outside Old Town, in neighborhoods like Dejvice, \\ Vinohrady, Holesovice, Karlin and New Town. Stop by for a coffee, hit up one of the many\\ great new bakeries or visit a charismatic old beer hall as you explore a city that is clearly \\ entering its prime.\end{tabular}                                                      & 110   \\ \cline{2-4} 
                                      & \begin{tabular}[c]{@{}l@{}}\href{https://cooking.nytimes.com/recipes/}{NYTimes}\\ (Food Writing)\end{tabular}           & \begin{tabular}[c]{@{}l@{}}The origins of the fruit sandwich are believed to go back to Japan’s luxury fruit stores and \\ the fruit parlors attached to them. This version comes from Yudai Kanayama, a native of \\ Hokkaido who runs the restaurants the Izakaya NYC and Dr Clark in New York. Fresh \\ fruit — fat strawberries, golden mango, kiwi with black ellipses of seeds, or whatever you\\ like — is engulfed in whipped cream mixed with mascarpone, which makes it implausibly \\ airy yet dense. (In Japanese, the texture is called fuwa-fuwa: fluffy like a cloud.) Pressed on\\ either side are crustless slices of shokupan, milk bread that agreeably springs back. The \\ sandwich looks like dessert but isn’t, or not exactly; it makes for a lovely little meal that \\ feels slightly illicit, as if for a moment there are no rules\end{tabular} & 83    \\ \cline{2-4} 
                                      & \begin{tabular}[c]{@{}l@{}}\href{https://www.nytimes.com/column/modern-love}{NYTimes}\\ (Personal Essay)\end{tabular}         & \begin{tabular}[c]{@{}l@{}}My dad’s Hinge profile showed his pandemic scruff, cheeky smirk and favorite frayed \\ T-shirt. He claimed his strength was listening but added the caveat that he ``may not agree\\ with you."He called it ``rugged charm"; I disagreed.After several matchless months, he let\\ me give his dating profile a millennial makeover. We swapped out his old photo for one of \\ him clean-shaven with a bright smile in the outdoors. We revamped his prompts to \\ highlight his superhero dad qualities and love of movies. My dad’s Hinge profile no longer\\ seemed unhinged. Two months later, he had a girlfriend.\end{tabular}                                                                                                                                                                                                            & 19    \\ \cline{2-4} 
                                      & \begin{tabular}[c]{@{}l@{}}\href{https://therumpus.net/sections/blogs/dear-sugar/}{Dear Sugar}\\ (Internet Advice)\end{tabular}     & \begin{tabular}[c]{@{}l@{}}What is a prestigious college? What did attending such a school allow you to believe about\\ yourself? What assumptions do you have about the colleges that you would not describe as\\ prestigious? What sorts of people go to prestigious colleges and not prestigious colleges?\\ Do you believe that you had a right to a free “first-rate” education? What do you make of the \\people who received educations that you would not characterize as first-rate? These are not \\rhetorical questions. I really do want you to take out a piece of paper and write those\\ questions down and then answer them. I believe your answers will deeply inform your current\\ struggle with jealousy. I am not asking you these questions in order to condemn or judge you.\\ I would ask a similar series of questions to anyone from any sort of background because I \\believe our early experiences and beliefs about our place in the world inform who [....]\\ \end{tabular}                                                                                                                                                                                                                                          & 30    \\ \hline
\end{tabular}
\vspace{2ex}
\caption{\label{table:source_paragraph}Venues of source material used to extract real-world examples of creative writing, used to prepare instructions for our experiments.}
\end{table*}
